Abelian 1-Calabi-Yau Categories

In this paper, we show all k-linear abelian 1-Calabi-Yau categories over an algebraically closed field k are derived equivalent to either the category of coherent sheaves on an elliptic curve, or to the finite dimensional representations of k[[t]]. Since all abelian categories derived equivalent with these two are known, we obtain a classification of all k-linear abelian 1-Calabi-Yau categories up to equivalence.

==> Abstract.tex <==
\begin{abstract}

\end{abstract}

==> Coherent.tex <==
\section{Coherent sequences}

Let $\AA$ be a connected $k$-linear abelian Ext-finite 1-Calabi-Yau category.  In this section, we wish to construct a derived equivalent category $\HH$ in which we may find a coherent and ample sequence in the sence of \cite{Polishchuk05}.  We start with some definitions.

\begin{definition}
\item A sequence $\EE = (E_i)_{i\in \bZ}$ is called \emph{projective} if for every epimorphism $X \to Y$ in $\HH$ there is an $n\in \bZ$ such that $\Hom(E_i,X) \to \Hom(E_i,Y)$ is surjective for $i < n$. 

\item A projective sequence $\EE = (E_i)_{i\in \bZ}$ is called \emph{coherent} if for every object $X \in \HH$ and $n \in \bZ$, there are integers $i_1, \ldots, i_s \leq n$ such that the canonical map
$$\bigoplus_{j=1}^s \Hom(E_i, E_{i_j}) \otimes \Hom(E_{i_j},X) \longrightarrow \Hom(E_i,X)$$
is surjective for $i<<0$.

\item A coherent and projective sequence $\EE =  (E_i)_{i\in \bZ}$ is \emph{ample} if for all $X \in \HH$ we have $\Hom(E_i,X) \not=0$ for $i<<0$.
\end{enumerate}
\end{definition}

With a sequence $$, we may associate an 
We wish to apply following theorem.

\begin{theorem}
Let 
\end{theorem}

\subsection{Preliminaries}

==> Main.tex <==

Let $\AA$ be an Ext-finite abelian 1-Calabi-Yau category and denote by $\CC$ the derived category $\Db \AA$.

\section{Endo-simple objects}

\begin{proposition}\label{proposition:EndoSimple}
Let $X$ be an object of $\AA$, then there exists an endo-simple object occurring both as subobject and quotient object of $X$.
\end{proposition}

\begin{proof}
Assume $X$ is not endo-simple and let $f : X \to X$ be a non-invertible endomorphism.  We show that $\dim \End I < \dim \End X$ where $I = \im f$.

Indeed, since we have an epimorphism $X \to I$ and monomorphism $I \to X$, we get a composition of monomorphisms $\Hom(I,I) \to \Hom(X,I) \to \Hom(X,X)$.  Since the image this composition has to be in $\rad(X,X)$, we know $\dim \Hom(I,I) < \dim \Hom(X,X)$.  Iteration finishes the proof.
\end{proof}

\begin{lemma}\label{lemma:CanonicalMap}
Let $A$ be an endo-simple object and $X \in \ind \AA$.  Each of the canonical maps $A \otimes \Hom(A,X) \longrightarrow X$ and $X \longrightarrow A \otimes \Hom(X,A)^\ast$ is either a monomorphism or an epimorphism.  If $\Hom(X,A) \not= 0$, then the first map is a monomorphism.  If $\Hom(A,X) \not= 0$, then the latter is an epimorphism.
\end{lemma}

\begin{proof}
Consider in the derived category $\Db \AA$ the twist functor $T_A$ characterized by
$$\tri {A \otimes \RHom(A,X)} X {T_A X}.$$
It is shown in \cite{Seidel01} that this is an equivalence.  Applying the homological functor $H^0$ gives the long exact sequence
$$0 \to H^{-1}(T_A X) \to A \otimes \Hom(A,X) \to X \to H^0(T_A X) \to A \otimes \Ext(A,X) \to 0$$
Since $X$ is incedomposable and $T_A$ is an equivalence, either $H^{-1}(T_A X)$ or $H^0(T_A X)$ is zero, hence the map is a monomorphism or an epimorphism, respectively.

If we assume furthermore $\Hom(X,A) \not= 0$, and hence by the Calabi-Yau property $\Ext(A,X) \not= 0$, we find $H^0(T_A X) \not= 0$.  Hence $H^{-1}(T_A X) = 0$ and the map $A \otimes \Hom(A,X) \to X$ is a monomorphism.

The other case is dual.
\end{proof}

\begin{proposition}\label{proposition:EndoSimplesDirected}
The subcategory of endo-simples is a directed category.
\end{proposition}

\begin{proof}
Let $A_0 \to A_1 \to \cdots \to A_n \to A_0$ be a cycle of non-zero non-isomorphisms between endo-simple objects.  We will assume $n$ is minimal with the property that such a cycle exists.

By Lemma \ref{lemma:CanonicalMap} we know that the canonical map $\phi:A_0 \otimes \Hom(A_0,A_1) \to A_1$ is either a monomorphism or an epimorphism.  If $\phi$ is a monomorphism, then we find a non-zero non-invertible morphism $A_n \to A_1$ and if $\phi$ is an epimorphism, we find a non-zero non-invertible morphism $A_0 \to A_2$.  In both cases we have found a shorter cycle, contradicting with the minimality of $n$.
\end{proof}

We now wish to show that every object has a composition series with endo-simple quotients.  Evenmoreso, every indecomposable object has a composition series in which only one isomorphism class of endo-simple objects occur as quotients.  We start with following lemma.

\begin{lemma}\label{lemma:Cone}
Let $X$ be an indecomposable object and $S$ an endo-simple object such that $\Hom(S,X) \not= 0$ and $\Hom(X,S) \not= 0$.  If $X$ is not isomorphic to $S$, then the cokernel $C$ of the canonical map $\varphi:S \otimes \Hom(S,X) \to X$ is indecomposable and $\dim \Hom(S,X) = \dim \Hom(S,C)$.
\end{lemma}

\begin{proof}
It will be convenient to work in the derived category $\Db \AA$.  Denote $V= \Hom(S,X)$ and consider the following triangle
$$\xymatrix@1{S \otimes V  \ar[r]^-{\varphi}& X \ar[r]& C \ar[r]^-{\psi} & S \otimes V [1]}.$$
Applying the functor $\Hom(-,S[1])$ to this triangle and using that for every non-zero map in $\Hom(S,S[1])$ composition with a non-split map gives zero, we see that every map $C \to S[1]$ factors through $\psi$.  Applying the functor $\Hom(S,-)$ shows $\dim \Hom(S,C) = \dim \Hom(S,S[1] \otimes V) = \dim \Hom(S,X)$.

Now, let $C_1$ be a direct summand of $C$ and let $\psi_1 : C \to S[1] \otimes \Hom(C_1,S[1])^{*}$ be the canonical map.  The following diagram commutes
$$
\xymatrix{S \otimes \Hom(C_1,S[1])^{*} \ar[r]\ar[d] & A \ar[r] & C_1 \ar[d]^{i}\ar[r]^-{\psi_1} & S[1] \otimes \Hom(C_1,S[1])^{*}\ar[d]^{i'} \\
S \otimes \Hom(S,X)  \ar[d]\ar[r]^-{\varphi}& X \ar[r]& C \ar[d]^{\pi}\ar[r]^-{\psi} & S \otimes \Hom(S,X)[1] \ar[d]^{\pi'}\\
S \otimes \Hom(C_1,S[1])^{*} \ar[r] & A \ar[r] & C_1 \ar[r]^-{\psi_1} & S[1] \otimes \Hom(C_1,S[1])^{*}
}
$$
where all rows are triangles, and where $\pi \circ i$ and $\pi' \circ i'$ are isomorphisms.  It now follows that $A$ is a direct summand of $X$.  Since $X$ is indecomposable, $A$ is either isomorphic to $X$ or to zero.  We conclude $C_1$ is isomorphic to a number of copies of $S[1]$ or to $C$. Since $C \in \AA[0]$ and $S[1] \in \AA[1]$ we may conclude $C_1 \cong C$ and hence $C$ is indecomposable.
\end{proof}

\begin{proposition}\label{proposition:Building}
Every indecomposable object is constructed by multiple extensions an endo-simple object with itself.
\end{proposition}

\begin{proof}
Let $S$ be an endo-simple object and denote by $\AA_S$ the full subcategory of $\AA$ spanned by the objects $Z$ which can be obtained from $S$ by taking a finite amount of extensions.  The number of such extensions needed, will be denoted by $l_S(Z)$, and we will refer to it as the lenght of $Z$.  We will prove that if $X$ is an indecomposable object of $\AA$ such that $S$ occurs both as quotient and subobject, then $X \in \AA_S$.

Since for every subobject $A$ of $X$ in $\AA_f$ of $X$ and quotient object $W$ of $X$ in $\AA_f$, we have
\begin{equation*}
\dim \End_\AA(X)\ge \sum_S \min (l_S(A),l_S(B)).
\end{equation*}
we may deduce either the lenght of such subobjects or the lenght of such quotient objects is bounded.  Assume the former, the latter is dual.

Let $A \in \AA_S$ be a subobject of $X$ such that $C = \coker(A \to X)$ is indecomposable and $\dim \Hom(S,C) \not= 0$, for example $A = 0$.  Since there is a bound on the lenght of subobjects of $X$ in $\AA_f$, we may furthermore assume $l_S(A)$ is maximal with these properties.  We wish to show that $C \cong S$.

It is easy to see that $\Hom(C,S) \not= 0$, hence by Lemma \ref{lemma:CanonicalMap} we know the canonical map $S \otimes \Hom(S,C) \longrightarrow C$ is a monomorphism.  Consider the commuting diagram with exact rows and columns
$$\xymatrix{
&& 0\ar[d] & 0\ar[d] & \\
0 \ar[r] & A \ar[r]\ar@{=}[d] & A' \ar[r]\ar[d] & S \otimes \Hom(S,C) \ar[r]\ar[d] & 0 \\
0 \ar[r] & A \ar[r] & X \ar[r]\ar[d] & C \ar[r]\ar[d] & 0 \\
&& C' \ar@{=}[r]\ar[d] & C' \ar[d] & \\
&& 0 & 0 &
}$$

If $C \not \cong S$, then by Lemma \ref{lemma:Cone}, we know $C'$ is indecomposable and $\dim \Hom(S,C') = \dim \Hom(S,C)$, yet $l_S(A') = l_S(A) + \dim \Hom(S,C)$, contradicting the maximality of $l_S(A)$.
\end{proof}

\section{Finding an ample sequence by twisting}\label{section:Ample}

In what follows, we will assume $A$ and $B$ are non-isomorphic endo-simples with $\dim \Hom(A,B) \not= 0$.  Denote $t = T_B$ and $t^n A = A_n$.

The following aisle will define a $t$-structure in $\CC$ with a hereditary heart $\HH$.
\begin{eqnarray*}
\ind D^{\leq 0} &=& \{X \in \ind \CC \mid \mbox{there is a path from $A_i$ to $X$, for an $i \in \bZ$}\} \\
\ind D^{\geq 1} &=& \ind \CC \setminus \ind D^{\leq 0}
\end{eqnarray*}

Recall the following definitions from \cite{Polishchuk05}.
\begin{enumerate}
\item A sequence $\EE = (E_i)_{i\in \bZ}$ is called \emph{projective} if for every epimorphism $X \to Y$ in $\HH$ there is an $n\in \bZ$ such that $\Hom(E_i,X) \to \Hom(E_i,Y)$ is surjective for $i < n$. 

\item A projective sequence $\EE = (E_i)_{i\in \bZ}$ is called \emph{coherent} if for every object $X \in \HH$ and $n \in \bZ$, there are integers $i_1, \ldots, i_s \leq n$ such that the canonical map
$$\bigoplus_{j=1}^s \Hom(E_i, E_{i_j}) \otimes \Hom(E_{i_j},X) \longrightarrow \Hom(E_i,X)$$
is surjective for $i<<0$.

\item A coherent and projective sequence $\EE =  (E_i)_{i\in \bZ}$ is \emph{ample} if for all $X \in \HH$ the map $\Hom(E_i,X) \not=0$ for $i<<0$.
\end{enumerate}

We now wish to show the sequence $\EE = (A_i)_{i \in \bZ}$ is projective, coherent and ample.  The following lemma will be useful.

\begin{lemma}
If $\Hom(A_i,X) \not=0$, then $\Hom(A_j,X) \not=0$ for all $j \leq i$.
\end{lemma}

\begin{proof}
It suffices to show that $\Hom(A_{i-1},X) \not=0$.  Since $\Hom(A_i,X) \not=0$ and $t$ is an auto-equivalence, we know $\Hom(A_{i-1,},t^-X) \not=0$.  Applying the functor $\Hom(A_{i-1},-)$ to the triangle
$$\xymatrix@1{B[-1] \otimes \Hom(X,B)^\ast \ar[r] & t^- X \ar[r] & X \ar[r] & B \otimes \Hom(X,B)^\ast}$$
and using $\Hom(A_{i-1}, B[-1])=0$ yields $\Hom(A_{i-1},X) \not= 0$.
\end{proof}

\begin{proposition}\label{proposition:EE}
In $\HH$ the sequence $\EE = (A_i)$ is projective, coherent and ample.
\end{proposition}

\begin{proof}
First, we will show $\EE$ is projective.  Therefore, let $X \to Y$ be an epimorphism and let $K$ be the kernel.  Since $K \in \HH$, we know there are paths from the sequence $\EE$ to every direct summand of $K$.  Hence $\Hom(K, A_i)=0$ for $i<<0$ and, by the Calabi-Yau property, $\Ext(A_i,K)=0$.  Thus $\Hom(A_i,X) \to \Hom(A_i,Y)$ is surjective for $i < n$.

Next, we will show $\EE$ is coherent.  For this, it will be convenient to work in the derived category.  The following two triangles in $\Db \HH$ will be used
\begin{equation}\label{equation:Triangle1}
\xymatrix@1{B \otimes V^\ast [-1] \ar[r]^-{\theta} & A_{i-1} \ar[r] & A_i \ar[r] & B \otimes V^\ast}
\end{equation}
and
\begin{equation}\label{equation:Triangle2}
\xymatrix@1{B \otimes V^\ast [-1] \ar[r]^-{\varphi} & A_{j} \ar[r] & A_{j+1} \ar[r] & B \otimes V^\ast}
\end{equation}
where $V = \Hom(A_i,B)$ and where we will assume $i<j$ has been chosen small enough such that $\Hom(A_{j+1},X) \not= 0$ for a chosen object $X$ in $\HH \subseteq \Db \HH$.  We will show a map $f: A_{i-1}\longrightarrow X$ factors through $A_i \oplus A_{j}$.

We may assume $f: A_{i-1}\longrightarrow X$ does not factor though $A_i$, hence from triangle (\ref{equation:Triangle1}) it follows that the composition $f \circ \theta \not= 0$.

Applying the functor $\Hom(-,X)$ on triangle (\ref{equation:Triangle2}) shows that every map $B \otimes V^\ast [-1] \longrightarrow X$ factors though $\varphi$.  Hence there is a morphism $g : A_{j} \longrightarrow X$ such that the following diagram commutes.
$$\xymatrix{
B \otimes V^\ast [-1] \ar[r]^-{\theta} \ar[d]_{\varphi}& A_{i-1} \ar[d]^f\\
A_{j} \ar[r]^-{g} & X
}$$

Furthermore, applying $\Hom(-,A_{j})$ to triangle (\ref{equation:Triangle1}) yields that $\varphi$ factors through $\theta$, hence there is a map $h : A_{i-1} \longrightarrow A_{j}$ such that $g \circ h \circ \theta = f \circ \theta$, or $(g \circ h - f) \circ \theta = 0$.

Summarizing, $f = g \circ j + f'$, where $f' : A_{i-1} \longrightarrow X$ lies in $\Ker(\theta,X)$ and as such factors through $A_i$.  The map $f$ factors though $A_i \oplus A_{j}$ and we may conclude the sequence $\EE$ is coherent.

Finally, we show the sequence $\EE$ is ample.  Let $X$ be an indecomposable object.  It suffices to prove that if $\Hom(A_n,X) \not= 0$, then there is a finite set $I \subset \bZ$ such that 
$$\bigoplus_{i\in I} A_i \otimes \Hom(A_i,X) \longrightarrow X$$
is an epimorphism.

So, let $i_1, \ldots, i_m \in \bZ$ be as in the definition of coherence.  Consider the map
\begin{equation}\label{equation:Ample}
\theta : \bigoplus_{j=1}^{m} A_{i_j} \otimes \Hom(A_{i_j},X) \longrightarrow X
\end{equation}
and let $C = \coker \theta$.  To ease notation, we will refer to the domain of $\theta$ by $\dom \theta$.  By the Calabi-Yau property, we may assume there is an $i_j$ such that $\Hom(A_{i_j}, C) \not= 0$.  Since $\EE$ is projective, there is a $k<<0$ such that the induced map in $\Hom(A_k,C)$ lifts to a map in $\Hom(A_k,X)$.  Again using coherence, this map should factor through $\dom \theta$.  We may conclude $C=0$.
\end{proof}

Denote by $R_m$ the abelian group $\Hom(A_0, A_m)$ and by $R$ the graded algebra $\oplus_m R_m$.  We will now proceed by describing the algebra $R = A(\EE)$.

\begin{lemma}\label{lemma:Domain}
Assume $A$ and $B$ have been chosen such that $n=\dim \Hom_{\Db \AA}(A,B)$ is minimal and $n \not= 0$.  Then $R$ is a domain.
\end{lemma}

\begin{proof}
It suffices to show every non-zero morphism $A_0 \longrightarrow A_j$ is a monomorphism.  Let $f : A_0 \longrightarrow A_i$ be a non-zero non-isomorphism.  We will show $f$ is a monomorphism.

We will prove this by induction on $i$.  The case $i=0$ is trivial.  So let $i \geq 1$.

Since $\im f$ is a quotient object of $A_0$ and $\dim \Hom(A,B)=n$, we see that $\dim \Hom(\im f, B) \leq n$, and due to the minimality of $n$, we know that either $\dim \Hom(\im f, B)=n$ or $\dim \Hom(\im f, B)=0$.

If $\dim \Hom(\im f, B)=0$, the inclusion $\im f \hookrightarrow A_i$ has to factor through an inclusion $j:\im f \hookrightarrow A_{i-1}$.

$$\xymatrix{
&&A_0 \ar@{->>}[d]\\
&&{\im f} \ar@{^{(}->}[d]\ar@{_{(}-->}[ld]_{\exist j}\\
0\ar[r]&A_{i-1}\ar[r]&A_i\ar[r]&B\otimes\Hom(A_i,B)^*\ar[r]&0}$$  

Composition gives a non-zero map $A_0 \longrightarrow A_{i-1}$ which is a monomorphism by the induction hypothesis.  We find that $A_0 \cong \im f$, hence $f$ is a monomorphism.

We are left with $\dim \Hom(\im f,B)=n$, and hence $\dim \Hom(K,B)=0$ where $K = \ker f$.  With $\EE$ being ample, we may assume there is a $k \in \bZ$, such that $A_k$ maps non-zero to every direct summand of $K$.  Using the exact sequence $0 \to A_k \to A_{k+1} \to B \otimes \Hom(A_{k+1},B)^* \to 0$, we find that for every $l \in \bZ$, $A_l$ maps non-zero to every direct summand of $K$.  Hence $\Hom(K,A_i) = 0$ and thus $K=0$.  We conclude that $f$ is a monomorphism.
\end{proof}

\begin{lemma}\label{lemma:Degree1}
The sequence $\EE^{(3)}=(A_{3k})_{k\in \bZ}$ is a projective, coherent and ample sequence.  Furthermore $R^{(3)} = A(\EE^{(3)})$ is generated in degree 1.
\end{lemma}

\begin{proof}
the sequence $\EE^{(3)}$ is projective and ample since $\EE$ is.  Coherence of $\EE^{(3)}$ may be shown as in the proof of Proposition \ref{proposition:EE}.

Next, we prove $R^{(3)}$ is generated in degree one.  Therefore, it suffices to show that for every $k>1$ every map $A_0 \to A_{3k}$ factors through the canonical map $\theta : A_0 \to A_3 \otimes \Hom(A_0,A_3)^\ast$.  We write $V = \Hom(A_0,A_3)$ and we consider the triangle
$$\xymatrix@1{C \ar[r] & {A_0} \ar[r]^-{\theta} & A_3 \otimes V^\ast \ar[r]& C[1]}$$
where $C = T_{A_3} A_0$.  Applying the functor $\Hom(-,A_{3k})$ to this triangle gives the exact sequence
$$\Hom(C[1],A_{3k}) \longrightarrow \Hom(A_3 \otimes V^\ast,A_{3k}) \longrightarrow \Hom(A_0,A_{3k}) \longrightarrow \Hom(C,A_{3k-1}).$$
We will now compute the dimensions of these vector spaces.  Note that it follows from the definition of $A_i$ that $\dim \Hom (A_i, A_j) = (j-i)n^2$ for $j>1$ where $n = \dim \Hom(A_0,B)$.

Since $\dim \Hom(A_0,A_{3k}) = (3k)n^2$ and $\dim \Hom(A_3 \otimes V^\ast,A_{3k-1}) = 9(k-1)n^4$, we may see $\Hom(C[1],A_{3k}) \not= 0$ and yet $A_{3k} \not\cong C[1]$.

Using Proposition \ref{proposition:EndoSimplesDirected}, we may see $\Hom(C,A_{3k})=0$ hence every map $A_0 \longrightarrow A_{3k}$ lifts through $\theta$ and the algebra $R^{(3)}$ is generated in degree one.
\end{proof}

We are now ready to prove our main theorem.

\begin{theorem}
Let $\AA$ be a connected $k$-linear abelian Ext-finite 1-Calabi-Yau category, then $\AA$ is derived equivalent to either
the category of finite dimensional nilpotent representations of $k[X]$ or the category of coherent sheaves on an elliptic curve $X$.
\end{theorem}

\begin{proof}
By Proposition \ref{proposition:EndoSimple} we know there are endo-simple objects.  If there is only one endo-simple object, $S$, then $\AA$ is noetherian and, by \cite{ReVdB02}, equivalent to the finite dimensional nilpotent representations of the one loop quiver.

If $\AA$ has at least two endo-simple objects, then we may chose two non-ismorphic endo-simples, $A$ and $B$, in $\Db \AA$ such that $\dim \Hom_{\Db \AA}(A,B)$ is minimal and non-zero.  Consider the abelian category $\HH$ constructed in \S\ref{section:Ample} with ample, coherent sequence $\EE^{(3)}$.

By Lemmas \ref{lemma:Domain} and \ref{lemma:Degree1}, we know $R^{(3)} = A(\EE^{(3)})$ is a domain of GK-dimension 2 which is finitely generated by elements of degree one, hence by \cite{Artin95} we find that $R^{(3)}$ is noetherian and $\qgr R^{(3)}$ is equivalent to the coherent sheaves on a curve $X$.

Since $R$ is noetherian, it follows from \cite{Polishchuk05} that $\HH$ is equivalent to $\qgr R^{(3)}$.

The structure sheaf $\OO_X$ corresponds to $A$.  Since the genus of $X$ is $\dim H^1(\OO_X) = \dim \Ext(\OO_X, \OO_X) = \dim \Ext(A,A) = 1$, we know that $X$ is an elliptic curve.
\end{proof}

==> Notations.tex <==
\section{Notations and conventions}

Throughout this paper, fix an algebraically closed field $k$ of arbitrary characteristic.  All algebras and categories are assumed to be $k$-linear.

%If $\mathfrak{a}$ is a small pre-additive category, we denote by $\Mod(\mathfrak{a})$ the abelian category of all left modules, thus all covariant functors from $\mathfrak{a}$ to $\Mod(k)$, the category of vectorspaces over $k$.  The category $\mod(\mathfrak{a})$ is the full subcategory of $\Mod(\mathfrak{a})$ consisting of finitely presented objects.  We will interpret an algebra as a pre-additive category consisting of one object.

%For a category $\CC$, we will write $\ind \CC$ for a chosen set of representatives of non-isomorphic indecomposable objects of $\CC$.  If $E$ is an object of $\CC$, then $\ind E$ is a chosen set of representatives of non-isomorphic indecomposable direct summands of $E$.

%The ring $\bZ$ is the ring of integers.  We will write $\bZz$ for $\bZ \setminus \{0\}$.

%If $\QQ$ is a quiver, a poset, an algebra, or more generally, a pre-additive category, we will write $\QQ^{\circ}$ for the dual quiver, poset, algebra, or pre-additive category.

%Given a category $\CC$, the \emph{Auslander-Reiten quiver of $\CC$} is defined as follows: the vertices of $\CC$ are the isomorphism classes  $[X]$ of indecomposable objects $X$.  There is an arrow $[X] \r [Y]$ if there is an irreducible morphism between $X \r Y$.  If $\KK$ is a component of the Auslander-Reiten quiver of $\CC$, also called an \emph{Auslander-Reiten component of $\CC$}, we will often, by abuse of notation, write $X \in \KK$ and $X = Y$, when we mean $[X] \in \KK$ and $[X] = [Y]$, respectively.

%For an abelian category or pre-additive category $\AA$, we will write $\Kb \AA$ for the category of bounded complexes modulo homotopy relations.

If $\AA$ is abelian, we write $\Db \AA$ for the bounded derived category of $\AA$.  The category $\Db \AA$ has the structure of a triangulated category.  Whenever we use the word "triangle" we mean "distinguished triangle".

%We will say a Krull-Schmidt abelian or triangulated category $\AA$ is \emph{connected} if for all $X, Y \in \ind \AA$ there is a finite, non-oriented path of non-zero morphisms between $X$ and $Y$ or between $X$ and $Y[z]$ for a $z \in \bZ$, respectively.

==> Tilting.tex <==
\section{Tilting}

In this section, we will give a description of all categories derived equivalent to an abelian 1-Calabi-Yau category.  In order to do this, we will use tilting in the sense of \cite{Happel96}.  We start with a short summary of some results.

Let $\AA$ be a hereditary abelian category.  A \emph{split torsion theory} on $\AA$, $(\FF,\TT)$ is a pair of full additive subcategories of $\AA$, such that $\Hom(\TT,\FF)=\Ext(\FF,\TT)=0$ and having the additional property that for every $X \in \Ob \AA$ there are objects $F \in \FF$ and $T \in TT$ such that $X \cong F \oplus T$.

We may then use tilting to obtain a hereditary category $\HH$ with an induced split torsion theory $(\TT,\FF[1])$.  The category $\HH$ is derived equivalent to $\AA$.



  We will call the objects of $\FF$ and $\TT$ the \emph{torsionfree objects} and the \emph{torsion objects}, respectively.

We will say $(\FF,\TT)$ is a split torsion theory if $\Ext(\FF,\TT)=0$.

If $\AA$ is an 1-Calabi-Yau category, then it follows from $\Hom(T,F)=0$ that every object in $\AA$ is a direct sum of object from $\FF$ and $\TT$.



In this section, we will give a description of all categories derived equivalent to an abelian 1-Calabi-Yau category.  Therefore, let $\AA$ be an abelian 1-Calabi-Yau category.  It follows from Theorem \ref{theorem:Main} that either $\AA$ is derived equivalent to $\Modfd k[[t]]$ or to $\coh X$ where $X$ is an elliptic curve.

By Proposition \ref{proposition:Dimension} we know that every category $\HH$ derived equivalent to $\AA$ is hereditary.  Hence, if $(D^{\geq 0}, D^{\leq 0})$ is a $t$-structure of $\Db \AA$ with $\HH$ as heart, then $(D^{\geq 0}, D^{\leq 0})$ is a split $t$-structure.  We may thus classify all possible $t$-structures on $\Db \AA$.

First, assume $\AA$ is equivalent to $\Modfd k[[t]]$, thus every two endo-simple objects in $\AA$ are isomorphic.  Let $(D^{\geq 0}, D^{\leq 0})$ be any $t$-structure.  Since this is split, there is an endo-simple $S$ from $\Db \AA$ in $\HH$.  Is readily follows from the definition that the only possible $t$-structure is
\begin{eqnarray*}
\ind D^{\leq 0} &=& \{X \in \ind \Db\AA \mid \mbox{there is a path from $S$ to $X$}\} \\
\ind D^{\geq 1} &=& \ind \Db \AA \setminus \ind D^{\leq 0}.
\end{eqnarray*}
We conclude that $\AA \cong \HH$.

We now consider the case where $\AA$ is equivalent to the category $\coh X$ where $X$ is an elliptic curve.  The categories derived equivalent to $\coh X$ have been described in \cite{}.  We may descrbie them as follows.

Let $\OO$ be the stucture sheaf and $k(P)$ be a torsion sheaf.  For a coherent sheaf $\FF$ we define the \emph{degree} and \emph{rank} to be 
\begin{eqnarray*}
\deg \FF &=& \chi (\OO,\FF) \\
\rk \FF &=& \chi(\FF,k(P)),
\end{eqnarray*}
respectively.  Furthemore, we define the \emph{slope} to be $\mu(\FF)=\frac{\deg \FF}{\rk \FF}$.  It is well-known that for two endo-simple coherent sheaves $\FF$ and $\GG$ we have $\dim \Hom(\FF,\GG)$


Let $\FF$ and $\GG$ be two stable sheaves.  It is well-known that


n this section, we wish to give a short discussion of the category of coherent sheaves $\coh X$ over an elliptic curve $X$.  An elliptic curve is a curve of genus 1.  In particular, $\AA = \coh X$ is a 1-Calabi-Yau category.

Let $\OO$ be the stucture sheaf and, for $P$ a point, let $k(P)$ be a torsion sheaf.  For a coherent sheaf $\FF$ we define the \emph{degree} and \emph{rank} to be 
\begin{eqnarray*}
\deg \EE &=& \chi (\OO,\EE) \\
\rk \EE &=& \chi(\EE,k(P)),
\end{eqnarray*}
respectively.  The Riemann-Roch theorem learns
\begin{equation}\label{equation:RR}
\chi(\EE,\FF) = \deg \FF \rk \EE - \deg \EE \rk \FF.\end{equation}

Furthemore, we define the \emph{slope} to be $\mu(\EE)=\frac{\deg \EE}{\rk \EE} \in \QQ\cup\{ \infty \}$.  A coherent sheaf $\FF$ is called \emph{stable} or \emph{semi-stable} if for every short exact sequence $0 \longrightarrow \EE \longrightarrow \FF \longrightarrow \GG \longrightarrow 0$ we have $\mu(\EE) \leq \mu(\FF)$ or $\mu(\EE) < \mu(\FF)$, respectivily.

It follows from the Harder-Narasimhan filtration of $\FF$ that every indecomposable coherent sheaf on $X$ is semi-stable.  Furthermore, the stable sheafs are exactly the endo-simple sheaves.  It follows from (\ref{equation:RR}) that, for non-isomorphic endo-simple sheaves $\EE$ and $\FF$, we have $\Hom(\EE,\FF) \not= 0$ if and only if $\mu(\EE) < \mu(\FF)$.

This leads us to a classification of all abelian categories, derived equivalent to $\AA$.  Therefore, we will first a description of tilting in the sense of \cite{Happel96}.

Let $\AA$ be a hereditary abelian category.  A \emph{split torsion theory} on $\AA$, $(\FF,\TT)$ is a pair of full additive subcategories of $\AA$, such that $\Hom(\TT,\FF)=\Ext(\FF,\TT)=0$ and having the additional property that for every $X \in \Ob \AA$ there are objects $F \in \FF$ and $T \in TT$ such that $X \cong F \oplus T$.

We may then use tilting to obtain a hereditary category $\HH$, derived equivalent to $\AA$, with an induced split torsion theory $(\TT,\FF[1])$.  We will proceed by discussing the possible split torsion theories on $\AA$.





  We will call the objects of $\FF$ and $\TT$ the \emph{torsionfree objects} and the \emph{torsion objects}, respectively.

We will say $(\FF,\TT)$ is a split torsion theory if $\Ext(\FF,\TT)=0$.

If $\AA$ is an 1-Calabi-Yau category, then it follows from $\Hom(T,F)=0$ that every object in $\AA$ is a direct sum of object from $\FF$ and $\TT$.



\subsection{Coherent sheaves over an elliptic curve}

In this section, we wish to give a short discussion of the category of coherent sheaves $\coh X$ over an elliptic curve $X$.  An elliptic curve is a curve of genus 1.  In particular, $\AA = \coh X$ is a 1-Calabi-Yau category.

Let $\OO$ be the stucture sheaf and, for $P$ a point, let $k(P)$ be a torsion sheaf.  For a coherent sheaf $\FF$ we define the \emph{degree} and \emph{rank} to be 
\begin{eqnarray*}
\deg \EE &=& \chi (\OO,\EE) \\
\rk \EE &=& \chi(\EE,k(P)),
\end{eqnarray*}
respectively.  The Riemann-Roch theorem learns
\begin{equation}\label{equation:RR}
\chi(\EE_1,\EE_2) = \deg \EE_2 \rk \EE_1 - \deg \EE_1 \rk \EE_2 .\end{equation}

Furthemore, we define the \emph{slope} to be $\mu(\EE)=\frac{\deg \EE}{\rk \EE} \in \QQ\cup\{ \infty \}$.  A coherent sheaf $\EE$ is called \emph{stable} or \emph{semi-stable} if for every short exact sequence $0 \longrightarrow \EE' \longrightarrow \EE \longrightarrow \EE'' \longrightarrow 0$ we have $\mu(\EE') \leq \mu(\EE)$ or $\mu(\EE') < \mu(\EE)$, respectivily.

It follows from the Harder-Narasimhan filtration of $\FF$ that every indecomposable coherent sheaf on $X$ is semi-stable.  Furthermore, the stable sheafs are exactly the endo-simple sheaves.  It follows from (\ref{equation:RR}) that, for non-isomorphic endo-simple sheaves $\EE_1$ and $\EE_2$, we have $\Hom(\EE_1,\EE_2) \not= 0$ if and only if $\mu(\EE_1) < \mu(\EE_2)$.

\subsection{Tilting}

We give a description of tilting in the sense of \cite{Happel96}.  Let $\AA$ be a hereditary abelian category.  A \emph{torsion theory} on $\AA$, $(\FF,\TT)$, is a pair of full additive subcategories of $\AA$, such that $\Hom(\TT,\FF)=0$ and having the additional property that for every $X \in \Ob \AA$ there is a short exact sequence
$$0 \longrightarrow F \longrightarrow X \longrightarrow T \longrightarrow 0$$
with $F \in \FF$ and $T \in TT$.

We will say the torsion theory $(\FF,\TT)$ is split if $\Hom(\FF,\TT)=0$.  We may now use tilting to obtain a hereditary category $\HH$ derived equivalent to $\AA$ with an induced split torsion theory $(\TT,\FF[1])$.

\subsection{Tilting the category $\coh X$}

We will proceed by giving all torsion theories on $\AA = \coh X$.  Note that, since $\AA$ is 1-Calabi-Yau, every torsion theory is a split one.

Let 
